A Quick Overview on the Quantum Control Approach to the Lambda Calculus

In this short overview, we start with the basics of quantum computing, explaining the difference between the quantum and the classical control paradigms. We give an overview of the quantum control line of research within the lambda calculus, ranging from untyped calculi up to categorical and realisability models. This is a summary of the last 10+ years of research in this area, starting from Arrighi and Dowek's seminal work until today.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Mauricio Ayala-Rinc\'on, Eduardo Bonelli (Eds.):
16th Logical \\ and Semantic Frameworks with Applications (LSFA 2021)\\
EPTCS 357, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.357.1}{10.4204/EPTCS.357.1}}

